Holistic Combination of Structural and Textual Code Information for Context based API Recommendation

Context based API recommendation is an important way to help developers find the needed APIs effectively and efficiently. For effective API recommendation, we need not only a joint view of both structural and textual code information, but also a holistic view of correlated API usage in control and data flow graph as a whole. Unfortunately, existing API recommendation methods exploit structural or textual code information separately. In this work, we propose a novel API recommendation approach called APIRec-CST (API Recommendation by Combining Structural and Textual code information). APIRec-CST is a deep learning model that combines the API usage with the text information in the source code based on an API Context Graph Network and a Code Token Network that simultaneously learn structural and textual features for API recommendation. We apply APIRec-CST to train a model for JDK library based on 1,914 open-source Java projects and evaluate the accuracy and MRR (Mean Reciprocal Rank) of API recommendation with another 6 open-source projects. The results show that our approach achieves respectively a top-1, top-5, top-10 accuracy and MRR of 60.3%, 81.5%, 87.7% and 69.4%, and significantly outperforms an existing graph-based statistical approach and a tree-based deep learning approach for API recommendation. A further analysis shows that textual code information makes sense and improves the accuracy and MRR. We also conduct a user study in which two groups of students are asked to finish 6 programming tasks with or without our APIRec-CST plugin. The results show that APIRec-CST can help the students to finish the tasks faster and more accurately and the feedback on the usability is overwhelmingly positive.

==> discussion.tex <==
First, it is difficult to perform completely accurate control and data flow analysis on any kind of code snippets.
We should make sure that most code snippets of usual and frequent used control and data flow can be analyzed accurately.
For example, we consider the control structures in Table~\ref{table:control statement rules} as usual and frequent used control structures.
Second, the textual information is helpful but the quality of it cannot be guaranteed.
Though we adopt two attention mechanisms to extract the meaningful semantics in the textual information as much as possible, it cannot completely eliminate the noise.
We need to analyze the quality of textual information during the data processing step in our future work.
Third, all projects in our code corpus written in Java.
For other languages, the way of constructing an API context graph might be different due to the different grammar rules and the model might not achieve as good results as Java projects.
In addition, all projects are open source, the results might not be generalized to industrial projects.
Fourth, all the testing instances are generated in an automatically way by removing APIs at arbitrary positions which may not reflect the truly programming scenarios.
However, we do a user study to further evaluate the ability of our model on real-world scenarios.
Finally, the baseline approach \GraLan~used in our evaluations may not be properly implemented.
However, we do a comparison of our re-implement \GraLan~with \GraLan~implemented in~\cite{ASE18RecRank} and find that our re-implement \GraLan~is comparable. 

